Self-Supervised Pretraining Improves Self-Supervised Pretraining

While self-supervised pretraining has proven beneficial for many computer vision tasks, it requires expensive and lengthy computation, large amounts of data, and is sensitive to data augmentation. Prior work demonstrates that models pretrained on datasets dissimilar to their target data, such as chest X-ray models trained on ImageNet, underperform models trained from scratch. Users that lack the resources to pretrain must use existing models with lower performance. This paper explores Hierarchical PreTraining (HPT), which decreases convergence time and improves accuracy by initializing the pretraining process with an existing pretrained model. Through experimentation on 16 diverse vision datasets, we show HPT converges up to 80x faster, improves accuracy across tasks, and improves the robustness of the self-supervised pretraining process to changes in the image augmentation policy or amount of pretraining data. Taken together, HPT provides a simple framework for obtaining better pretrained representations with less computational resources.

==> coco_results_table.tex <==
\newcommand{\randinit}{\tablestyle{1pt}{1} \begin{tabular}{z{21}y{26}} \multicolumn{2}{c}{\demph{random init.}} \end{tabular}}
\renewcommand{\res}[3]{
\tablestyle{1pt}{1}
\begin{tabular}{z{14}y{18}}
{#1} &
\fontsize{7.5pt}{1em}\selectfont{(${#2}${#3})}
\end{tabular}}

\renewcommand{\reshl}[3]{
\tablestyle{1pt}{1}
\begin{tabular}{z{14}y{18}}
{#1} &
\fontsize{7.5pt}{1em}\selectfont{\textcolor{Highlight}{(${#2}$\textbf{#3})}} 
\end{tabular}}

\renewcommand{\resrand}[2]{\tablestyle{1pt}{1} \begin{tabular}{z{14}y{18}} \demph{#1} & {} \end{tabular}}
\renewcommand{\ressup}[2]{\tablestyle{1pt}{1} \begin{tabular}{z{14}y{18}} {#1} & {} \end{tabular}}


\newcommand{\cgap}[2]{
\fontsize{6pt}{1em}\selectfont{(${#1}${#2})}
}
\newcommand{\cgaphl}[2]{
\fontsize{6pt}{1em}\selectfont{\textcolor{Highlight}{(${#1}$\textbf{#2})}}
}

\renewcommand{\randinit}{\tablestyle{1pt}{1} \begin{tabular}{z{21}y{26}} \multicolumn{2}{c}{random init.} \end{tabular}}

\begin{table*}[ht]
	\small
	\resizebox{1.0\linewidth}{!}{
		\subfloat[Mask R-CNN R50-FPN, 1$\x$ schedule]{
			\tablestyle{.8pt}{1.05}
			\begin{tabular}{cr|
					z{17}y{18}
					z{17}y{18}
					z{17}y{18}|
					z{17}y{18}
					z{17}y{18}
					z{17}y{18}c
				}
				pretrain & ~ &
				\multicolumn{2}{c}{\apbbox{~}} &
				\multicolumn{2}{c}{\apbbox{50}} &
				\multicolumn{2}{c|}{\apbbox{75}} &
				\multicolumn{2}{c}{\apmask{~}} &
				\multicolumn{2}{c}{\apmask{50}} &
				\multicolumn{2}{c}{\apmask{75}} &\\
				\shline
				\demph{random init} & ~ &
				\demph{31.0} & ~ & \demph{49.5} & ~ & \demph{33.2} & ~ &
				\demph{28.5} & ~ & \demph{46.8} & ~ & \demph{30.4} & ~ & \\

				Base & ~ &
				38.9 & \cgap{+}{0.0} & 59.2 & \cgap{-}{0.4} & 42.4 & \cgap{-}{0.3} &
				35.4 & \cgap{+}{0.0} & 56.2 & \cgap{-}{0.3} & 37.8 & \cgap{-}{0.3} \\	
				
				HPT: Base-Target & ~ &
				38.9 & \cgap{+}{0.0} & 59.2 & \cgap{-}{0.4} & 42.4 & \cgap{-}{0.3} &
				35.4 & \cgap{+}{0.0} & 56.2 & \cgap{-}{0.3} & 37.8 & \cgap{-}{0.3} \\
			\end{tabular}	
		}  
		\subfloat[Mask R-CNN R50-FPN, 2$\x$ schedule]{
		\tablestyle{.8pt}{1.05}
			\begin{tabular}{
					z{17}y{18}
					z{17}y{18}
					z{17}y{18}|
					z{17}y{18}
					z{17}y{18}
					z{17}y{18}c
				}
				\multicolumn{2}{c}{\apbbox{~}} &
				\multicolumn{2}{c}{\apbbox{50}} &
				\multicolumn{2}{c|}{\apbbox{75}} &
				\multicolumn{2}{c}{\apmask{~}} &
				\multicolumn{2}{c}{\apmask{50}} &
				\multicolumn{2}{c}{\apmask{75}} &\\
				\shline
				\demph{36.7} & ~ & \demph{56.7} & ~ & \demph{40.0} & ~ & 
				\demph{33.7} & ~ & \demph{53.8} & ~ & \demph{35.9} & ~ &\\					
				40.6 & ~ & 61.3 & ~ & 44.4 & ~ &
				36.8 & ~ & 58.1 & ~ & 39.5 & ~ & \\

				40.9 & \cgap{+}{0.3} & 61.5 & \cgap{+}{0.2} & 44.6 & \cgap{+}{0.2} &
				37.0 & \cgap{+}{0.2} & 58.4 & \cgap{+}{0.3} & 39.6 & \cgap{+}{0.1} \\
				
				- &  & - &   & - &   &
				- &  & - &   & - &   & \\

				41.2 & \cgaphl{+}{0.6} & 61.9 & \cgaphl{+}{0.6} & 45.1 & \cgaphl{+}{0.7} &
				37.3 & \cgaphl{+}{0.5} & 58.9 & \cgaphl{+}{0.8} & 40.1 & \cgaphl{+}{0.6} \\\hline
				41.1 & \cgaphl{+}{0.5} & 61.5 & \cgap{+}{0.2} & 44.8 & \cgap{+}{0.4} &
				37.1 & \cgap{+}{0.3} & 
				58.6 & \cgaphl{+}{0.5} & 
				39.8 & \cgap{+}{0.3} \\
				
				\textbf{41.4} & \cgaphl{+}{0.8} & 61.8 & \cgaphl{+}{0.5} & 45.4 & \cgaphl{+}{1.0} &
				\textbf{37.5} & \cgaphl{+}{0.7} & \textbf{59.1} & \cgaphl{+}{1.0} & \textbf{40.4} & \cgaphl{+}{0.9} \\
				
				\textbf{41.4} & \cgaphl{+}{0.8} & \textbf{61.9} & \cgaphl{+}{0.6} & \textbf{45.4}  & \cgaphl{+}{1.0} &
				\textbf{37.5} & \cgaphl{+}{0.7} & \textbf{59.1} & \cgaphl{+}{1.0} & 40.3 & \cgaphl{+}{0.8} \\
			\end{tabular}	
		}  
	} 
    \vspace{0.1mm}
	\caption{\textbf{Results on COCO object detection and instance segmentation tasks.} The models are pre-trained on IN-1K for 200 epochs, the weights of which are transferred to Mask R-CNN R50-FPN model, subsequently finetuned on~\texttt{train2017} (1$\x$ and 2$\x$ schedules) and evaluated on~\texttt{val2017}. Averaging precision on bounding-boxes (AP$^{\text{bb}}$) and masks (AP$^{\text{mk}}$) are used as benchmark metrics. All \ours models outperform VADeR~\cite{pinheiro2020unsupervised} and the MoCo-v2 counterpart, surpassing the supervised pre-training under all metrics (we report VADeR results from their paper which did not include a 2x schedule). In the brackets are the gaps to the ImageNet supervised pre-training baseline. \textcolor{Highlight}{\textbf{Green}}: deltas at least +0.5. $^\dagger$: Pre-trained weights are downloaded from the official releases of the authors and trained on our COCO frameworks, as~\cite{wang2020dense} adopted a different COCO finetuning baseline settings from the common approach used in this paper and other previous works~\cite{he2019momentum}.
	}\vspace{-3.0mm}
	\label{tab:coco}
\end{table*}


==> expanded-related-work.tex <==
\section{Expanded Related Work}
\subsection{Source Model Selection/Transferability Estimation}
In this section, we discuss how HPT could be incorporated with transferability measures. Predicting the performance of transfer learning algorithms between two tasks is also addressed as transferability estimation~\cite{bao2019information, tran2019transferability}. It's vital since we hope to select the best performing source pre-trained model on the target task. One trivial approach, fine-tuning all models to find the best performing one is rapidly becoming computationally infeasible with increasing amount of data. Early theoretical works studied the \emph{relatedness} between tasks and proposed several types of distances, including $\mathcal{F}$-relatedness~\cite{ben2003exploiting}, $\mathcal{A}$-distance~\cite{kifer2004detecting, ben2007analysis}, and discrepancy distance~\cite{mansour2009domain}. More recent works developed transferability measures such as the negative conditional entropy measure~\cite{tran2019transferability}, or log expected empirical prediction (LEEP)~\cite{nguyen2020leep}. LEEP indicates the closeness of learned representation and target data whereby is utilized to measure the quality of representation learned using HPT or different pre-training methods from source data to target data. we will leave more details and quantitative analysis for future consideration.

\subsection{Adapting to Unseen Data}
Adapting to unseen data has been tackled from various perspectives in computer vision. Depending on the availability of the labeled data for the downstream task, some approaches (i) add a limited number of parameters to accompany new tasks and either train only the newly added parameters~\cite{va,efficient-va} or the entire network on the downstream task~\cite{expert-va}, or (ii) only train subparts of the network~\cite{schneider2020improving,nado2020evaluating} without using the labels of the target task. 
For the first type of approaches, visual adapters were proposed by~\cite{va} to adapt models across domains by adding a few trainable parameters called \textit{adapter modules}. Adapter modules can be trained solely~\cite{va,efficient-va} or along with the remaining of the network~\cite{expert-va} on the downstream task. If trained alone, tuning adapters can reduce training parameters by two orders of magnitude while maintaining similar performance as finetuning~\cite{nlp-adapters}. \cite{efficient-va} explored various techniques for designing efficient adapters and recently~\cite{expert-va} developed an adapter-based architecture to compress many experts into a single model where transfer to the downstream task is achieved by finetuning the entire expert network including the adapters. On the other hand, for the second line of approaches, one of the simplest yet strongest  is  updating batch normalization~\cite{bn} statistics at test-time which does not require labels for the target task~\cite{schneider2020improving,nado2020evaluating}. \cite{tent} extended this direction and proposed test-time entropy minimization (tent) to learn normalization statistics and channel-wise affine transformation parameters using entropy as an unsupervised objective. Although tent is shown to outperform batchnorm finetuning~\cite{tent} and does not use labels at adaptation time, it requires class predictions for a supervised task which makes it inapplicable in scenarions such as HPT where the adaptation must be performed on a self-supervised task. Therefore, in our study we have adopted simple approach of batchnorm finetuning as follows: during the self-supervised pretraining phase we freeze all parameters excluding batchnorm layers whereas during the linear finetuning phase on the target task, we freeze all parameters including batchnorm layers. 

\subsection{Sequential Transfer Learning}
Transitive Transfer Learning \cite{TanTransitive} seeks to bridge a source domain with a target domain through a two step process where first, an intermediate domain is selected, and secondly, that domain is used for transitive knowledge transfer. 

They begin with a source dataset $S$, and target dataset $T$, and seek to find an intermediate dataset $D$ for knowledge transfer.  Selection of $D$ is done by evaluating various datasets. To begin, they measure the complexity of each dataset, and the distances between them. They then use these $6$ features as inputs to a logistic regression problem to see if the intermediate dataset $D$ helps bridge $S$ and $T$. They get labels for this by measuring semi supervised label propogation algorithm with $S$ and $T$, vs with $S$, $D$, and $T$. If the accuracy obtained on this task with with $S,D, T$ is greater than  accuracy with just $S,T$ then label is 1, otherwise 0. 

The learned regression function is then used to select the best intermediate dataset. Now that an intermediate dataset has been selected, they do transitive knowledge transfer. This is a non-negative matrix tri-factorization (NMTF) based method where they are doing self-supervised label propagation. The key here is that they use NMTF with two datasets at once (either $S$ and $D$ or $D$ and $T$), and force feature clustering factors to be shared between $S$ and $D$, and between $D$ and $T$. Furthermore, they find that if the self-supervised label matrix is shared for when they are doing NMTF between $S$ and $D$, \emph{and} $D$ and $T$, representations from the source domain can help those in the target domain through the intermediate domain. 

While they only evaluate primarily on binary classification tasks they showed strong results compared to other methods at the time. 


\subsection{HPT in other Applications}
Self-supervised learning through pretext tasks has experienced rapid adoption in the NLP community. As such, significant work has gone into adapting language models to novel tasks and domains. Most similar to our line of exploration is the recent work from Gururangan et.~al.'s~\cite{gururangan2020don} work on Domain-Adaptive Pretraining. They explore the effect of various forms of adaptively pretraining language models on domains closely related to the task of interest. However, they do not compare performance versus pretraining from scratch on the desired domain nor do they propose a strategy for limiting to parameters tuned during adaptive pretraining. Various other works in NLP literature use lightweight Adapter models \cite{pfeiffer2020adapterhub} to restrict the number of parameters updated during transfer learning while achieving strong performance. These approaches use small neural networks as opposed to updated the BatchNorm parameters as in our work.  

